From Innovations to Prospects: What Is Hidden Behind Cryptocurrencies?

The great influence of Bitcoin has promoted the rapid development of blockchain-based digital currencies, especially the altcoins, since 2013. However, most altcoins share similar source codes, resulting in concerns about code innovations. In this paper, an empirical study on existing altcoins is carried out to offer a thorough understanding of various aspects associated with altcoin innovations. Firstly, we construct the dataset of altcoins, including source code repositories, GitHub fork relations, and market capitalizations (cap). Then, we analyze the altcoin innovations from the perspective of source code similarities. The results demonstrate that more than 85% of altcoin repositories present high code similarities. Next, a temporal clustering algorithm is proposed to mine the inheritance relationship among various altcoins. The family pedigrees of altcoin are constructed, in which the altcoin presents similar evolution features as biology, such as power-law in family size, variety in family evolution, etc. Finally, we investigate the correlation between code innovations and market capitalization. Although we fail to predict the price of altcoins based on their code similarities, the results show that altcoins with higher innovations reflect better market prospects.

==> 8-Acknowledgment.tex <==
\section*{Acknowledgment}

This work was supported by National Key R\&D Program of China (2016YFB1000903), National Natural Science Foundation of China (61902306, 61632015, 61772408, U1766215, 61721002, 61532015, 61833015), Ministry of Education Innovation Research Team (IRT\_17R86), China postdoctoral science special foundation (No. 2019TQ0251), and Project of China Knowledge Centre for Engineering Science and Technology. Ting Liu is the corresponding author.
